Hard scattering cross sections at LHC in the Glauber approach: from pp to pA and AA collisions

The scaling rules of the invariant yields and cross sections for hard scattering processes in proton-nucleus ($pA$) and nucleus-nucleus ($AB$) reactions at LHC energies relative to those of nucleon-nucleon $NN$ (isospin averaged $pp$) collisions are reviewed within the Glauber geometrical formalism. The number of binary inelastic collisions for different centrality classes in p+Pb and Pb+Pb collisions at $\sqrt{s_{NN}}$ = 8.8 TeV and 5.5 TeV respectively, as obtained from a Glauber Monte Carlo, are also given.

==> sec11_bibli.tex <==
%%%
%%%%%% Bibliography from sec. 11: Appendices 
%%%

\bibitem{enterria:glau} R.J.~Glauber and G.~Matthiae, Nucl.\ Phys.\ B {\bf
21} (1970) 135. For a recent application of the Glauber approach to $pA$
collisions see e.g. T.~Wibig and D.~Sobczynska, J. Phys. G: Nucl. Part. Phys.
{\bf 24} (1998) 2037.
%; and in  JHEP 0209:015,2002 for hadron-hadron interactions.

\bibitem{enterria:deJae} C.W.~deJager, H.~deVries, and C.~deVries, Atomic
Data and Nuclear Data Tables {\bf 14} (1974) 485. 

\bibitem{NNcross-section} The values of $\sigma_{\mbox{\scriptsize{\it{NN}}}}$
at  $\sqrt{s_{\mbox{\scriptsize{\it{NN}}}}}$ = 5.5 TeV and  $\sqrt{s_{\mbox{\scriptsize{\it{NN}}}}}$ = 8.8 TeV
have been obtained from {\sc Dpmjet}. In this model the scattering amplitude is parametrized using 
${\sigma}_{tot}$, $\rho$ = ${\bf Re} f(0)_{hN}$/${\bf Im} f(0)_{hN}$ and the elastic slope $a$.
These parameters are taken as fitted by the {\sc Phojet} model \cite{phojet-a} and e.g. this gives at 5.5 TeV 
${\sigma}_{tot}$ = 101.13 mb, $\rho $ = 0.1 and $a$ = 18.26 GeV${}^2$.  From this the inelastic 
cross section ${\sigma }_{NN}^{inel}$ = 72.03 mb  is obtained.

\bibitem{pPbcross-section} The value $\sigma_{\mbox{\scriptsize{\it{pPb}}}}^{geo} \approx$ 2162 mb is
obtained directly from the Glauber model for $\sigma_{\mbox{\scriptsize{\it{NN}}}}$ = 77 mb.

\bibitem{PbPbcross-section} The value $\sigma_{\mbox{\scriptsize{\it{PbPb}}}}^{geo} \approx$ 7745 mb is
obtained directly from the Glauber model for $\sigma_{\mbox{\scriptsize{\it{NN}}}}$ = 72 mb.

\bibitem{enterria:vogt} R.~Vogt, Heavy Ions Physics {\bf 9} (1974) 399.
nucl-th/9903051.

\bibitem{enterria:star} P.~Jacobs and G.~Cooper, nucl-ex/0008015.

\bibitem{enterria:klaus} K.~Reygers, PHENIX Glauber MC. 
\scriptsize{$http://www.phenix.bnl.gov/software/cvsweb/cvsweb.cgi/offline/analysis/glauber\_mc$}.

%\bibitem{enterria:shmakov} S.Y.Shmakov et al., Comput, Phys. Commun. {\bf 54} (1989) 125.

%\bibitem{enterria:engel} R.Engel, Z. Phys. C {\bf 66} (1995) 203.%

